Warm-starting Contextual Bandits: Robustly Combining Supervised and Bandit Feedback

We investigate the feasibility of learning from a mix of both fully-labeled supervised data and contextual bandit data. We specifically consider settings in which the underlying learning signal may be different between these two data sources. Theoretically, we state and prove no-regret algorithms for learning that is robust to misaligned cost distributions between the two sources. Empirically, we evaluate some of these algorithms on a large selection of datasets, showing that our approach is both feasible and helpful in practice.

==> temp_fig.tex <==
\begin{figure}[H]
	%\vskip -100pt
\centering
\begin{tabular}{c | @{}c@{ }c@{ }c@{}} % trim={left lower right upper}
\toprule
& \multicolumn{3}{c}{ Ratio }
\\
Noise & 2.875 & 5.75 & 11.5
\\\midrule
Noiseless & \includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=1,cpws=0.0,cti=1,cpi=0.0},inter_ws_size_ratio={2.875},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=1,cpws=0.0,cti=1,cpi=0.0},inter_ws_size_ratio={5.75},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=1,cpws=0.0,cti=1,cpi=0.0},inter_ws_size_ratio={11.5},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
\\\hline
\begin{tabular}{c}UAR \\ $p=0.25$\end{tabular}
& \includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=1,cpws=0.25,cti=1,cpi=0.0},inter_ws_size_ratio={2.875},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=1,cpws=0.25,cti=1,cpi=0.0},inter_ws_size_ratio={5.75},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=1,cpws=0.25,cti=1,cpi=0.0},inter_ws_size_ratio={11.5},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
\\\hline
\begin{tabular}{c}MAJ \\ $p=0.25$\end{tabular}
& \includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=3,cpws=0.25,cti=1,cpi=0.0},inter_ws_size_ratio={2.875},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=3,cpws=0.25,cti=1,cpi=0.0},inter_ws_size_ratio={5.75},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=3,cpws=0.25,cti=1,cpi=0.0},inter_ws_size_ratio={11.5},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
\\\hline
\begin{tabular}{c}CYC \\ $p=0.25$\end{tabular}
& \includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=2,cpws=0.25,cti=1,cpi=0.0},inter_ws_size_ratio={2.875},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=2,cpws=0.25,cti=1,cpi=0.0},inter_ws_size_ratio={5.75},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=2,cpws=0.25,cti=1,cpi=0.0},inter_ws_size_ratio={11.5},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
\\\hline
\begin{tabular}{c}UAR \\ $p=0.5$\end{tabular}
& \includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=1,cpws=0.5,cti=1,cpi=0.0},inter_ws_size_ratio={2.875},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=1,cpws=0.5,cti=1,cpi=0.0},inter_ws_size_ratio={5.75},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=1,cpws=0.5,cti=1,cpi=0.0},inter_ws_size_ratio={11.5},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
\\\bottomrule
\multicolumn{4}{c}{
		\begin{subfigure}[t]{\textwidth}
			%\hspace{-1.3cm} for 1.2
    \includegraphics[width=\textwidth,trim={0 0 0 0},clip]{figs/cdfs/legends/legend_Lambda=8.pdf}
		\end{subfigure} }
\end{tabular}
\caption{Cumulative distribution functions (CDFs) for all evaluated algorithms, against different noise settings and warm start ratios in $\cbr{2.875,5.75,11.5}$. All CB algorithms uses $\epsilon$-greedy with $\epsilon=0.1$. In each of the above plots, the $x$ axis represents scores, while the $y$ axis represents the CDF values.}
\label{fig:cdfs-eps=0.1-1}
\end{figure}


\begin{figure}[H]
	%\vskip -100pt
\centering
\begin{tabular}{c | @{}c@{ }c@{ }c@{}} % trim={left lower right upper}
\toprule
& \multicolumn{3}{c}{ Ratio }
\\
Noise & 23.0 & 46.0 & 92.0
\\\midrule
Noiseless & \includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=1,cpws=0.0,cti=1,cpi=0.0},inter_ws_size_ratio={23.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=1,cpws=0.0,cti=1,cpi=0.0},inter_ws_size_ratio={46.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=1,cpws=0.0,cti=1,cpi=0.0},inter_ws_size_ratio={92.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
\\\hline
\begin{tabular}{c}UAR \\ $p=0.25$\end{tabular}
& \includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=1,cpws=0.25,cti=1,cpi=0.0},inter_ws_size_ratio={23.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=1,cpws=0.25,cti=1,cpi=0.0},inter_ws_size_ratio={46.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=1,cpws=0.25,cti=1,cpi=0.0},inter_ws_size_ratio={92.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
\\\hline
\begin{tabular}{c}MAJ \\ $p=0.25$\end{tabular}
& \includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=3,cpws=0.25,cti=1,cpi=0.0},inter_ws_size_ratio={23.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=3,cpws=0.25,cti=1,cpi=0.0},inter_ws_size_ratio={46.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=3,cpws=0.25,cti=1,cpi=0.0},inter_ws_size_ratio={92.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
\\\hline
\begin{tabular}{c}CYC \\ $p=0.25$\end{tabular}
& \includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=2,cpws=0.25,cti=1,cpi=0.0},inter_ws_size_ratio={23.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=2,cpws=0.25,cti=1,cpi=0.0},inter_ws_size_ratio={46.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=2,cpws=0.25,cti=1,cpi=0.0},inter_ws_size_ratio={92.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
\\\hline
\begin{tabular}{c}UAR \\ $p=0.5$\end{tabular}
& \includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=1,cpws=0.5,cti=1,cpi=0.0},inter_ws_size_ratio={23.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=1,cpws=0.5,cti=1,cpi=0.0},inter_ws_size_ratio={46.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=1,cpws=0.5,cti=1,cpi=0.0},inter_ws_size_ratio={92.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
\\\bottomrule
\multicolumn{4}{c}{
		\begin{subfigure}[t]{\textwidth}
			%\hspace{-1.3cm} for 1.2
    \includegraphics[width=\textwidth,trim={0 0 0 0},clip]{figs/cdfs/legends/legend_Lambda=8.pdf}
		\end{subfigure} }
\end{tabular}
\caption{Cumulative distribution functions (CDFs) for all evaluated algorithms, against different noise settings and warm start ratios in $\cbr{23.0,46.0,92.0}$. All CB algorithms uses $\epsilon$-greedy with $\epsilon=0.1$. In each of the above plots, the $x$ axis represents scores, while the $y$ axis represents the CDF values.}
\label{fig:cdfs-eps=0.1-2}
\end{figure}

\begin{figure}[H]
	%\vskip -100pt
\centering
\begin{tabular}{c |@{}c@{}} % trim={left lower right upper}
\toprule
& \multicolumn{1}{c}{ Ratio }
\\
Noise & 184.0
\\\midrule
Noiseless & \includegraphics[width=0.3\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=1,cpws=0.0,cti=1,cpi=0.0},inter_ws_size_ratio={184.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
\\\hline
\begin{tabular}{c}UAR \\ $p=0.25$\end{tabular}
& \includegraphics[width=0.3\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=1,cpws=0.25,cti=1,cpi=0.0},inter_ws_size_ratio={184.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}

\\\hline
\begin{tabular}{c}MAJ \\ $p=0.25$\end{tabular}
& \includegraphics[width=0.3\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=3,cpws=0.25,cti=1,cpi=0.0},inter_ws_size_ratio={184.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}

\\\hline
\begin{tabular}{c}CYC \\ $p=0.25$\end{tabular}
& \includegraphics[width=0.3\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=2,cpws=0.25,cti=1,cpi=0.0},inter_ws_size_ratio={184.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}

\\\hline
\begin{tabular}{c}UAR \\ $p=0.5$\end{tabular}
& \includegraphics[width=0.3\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=1,cpws=0.5,cti=1,cpi=0.0},inter_ws_size_ratio={184.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}

\\\bottomrule
\multicolumn{2}{c}{
		\begin{subfigure}[t]{\textwidth}
			%\hspace{-1.3cm} for 1.2
    \includegraphics[width=\textwidth,trim={0 0 0 0},clip]{figs/cdfs/legends/legend_Lambda=8.pdf}
		\end{subfigure} }
\end{tabular}
\caption{Cumulative distribution functions (CDFs) for all evaluated algorithms, against different noise settings and warm start ratios in $\cbr{184.0}$. All CB algorithms uses $\epsilon$-greedy with $\epsilon=0.1$. In each of the above plots, the $x$ axis represents scores, while the $y$ axis represents the CDF values.}
\label{fig:cdfs-eps=0.1-3}
\end{figure}

\begin{figure}[H]
	%\vskip -100pt
\centering
\begin{tabular}{c | @{}c@{ }c@{ }c@{}} % trim={left lower right upper}
\toprule
& \multicolumn{3}{c}{ Ratio }
\\
Noise & 2.875 & 5.75 & 11.5
\\\midrule
\begin{tabular}{c}MAJ \\ $p=0.5$\end{tabular}
 & \includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=3,cpws=0.5,cti=1,cpi=0.0},inter_ws_size_ratio={2.875},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=3,cpws=0.5,cti=1,cpi=0.0},inter_ws_size_ratio={5.75},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=3,cpws=0.5,cti=1,cpi=0.0},inter_ws_size_ratio={11.5},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
\\\hline
\begin{tabular}{c}CYC \\ $p=0.5$\end{tabular}
& \includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=2,cpws=0.5,cti=1,cpi=0.0},inter_ws_size_ratio={2.875},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=2,cpws=0.5,cti=1,cpi=0.0},inter_ws_size_ratio={5.75},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=2,cpws=0.5,cti=1,cpi=0.0},inter_ws_size_ratio={11.5},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
\\\hline
\begin{tabular}{c}UAR \\ $p=1$\end{tabular}
& \includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=1,cpws=1.0,cti=1,cpi=0.0},inter_ws_size_ratio={2.875},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=1,cpws=1.0,cti=1,cpi=0.0},inter_ws_size_ratio={5.75},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=1,cpws=1.0,cti=1,cpi=0.0},inter_ws_size_ratio={11.5},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
\\\hline
\begin{tabular}{c}MAJ \\ $p=1$\end{tabular}
& \includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=3,cpws=1.0,cti=1,cpi=0.0},inter_ws_size_ratio={2.875},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=3,cpws=1.0,cti=1,cpi=0.0},inter_ws_size_ratio={5.75},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=3,cpws=1.0,cti=1,cpi=0.0},inter_ws_size_ratio={11.5},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
\\\hline
\begin{tabular}{c}CYC \\ $p=1$\end{tabular}
& \includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=2,cpws=1.0,cti=1,cpi=0.0},inter_ws_size_ratio={2.875},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=2,cpws=1.0,cti=1,cpi=0.0},inter_ws_size_ratio={5.75},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=2,cpws=1.0,cti=1,cpi=0.0},inter_ws_size_ratio={11.5},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
\\\bottomrule
\multicolumn{4}{c}{
		\begin{subfigure}[t]{\textwidth}
			%\hspace{-1.3cm} for 1.2
    \includegraphics[width=\textwidth,trim={0 0 0 0},clip]{figs/cdfs/legends/legend_Lambda=8.pdf}
		\end{subfigure} }
\end{tabular}
\caption{Cumulative distribution functions (CDFs) for all evaluated algorithms, against different noise settings and warm start ratios in $\cbr{2.875,5.75,11.5}$. All CB algorithms uses $\epsilon$-greedy with $\epsilon=0.1$. In each of the above plots, the $x$ axis represents scores, while the $y$ axis represents the CDF values.}
\label{fig:cdfs-eps=0.1-4}
\end{figure}

\begin{figure}[H]
	%\vskip -100pt
\centering
\begin{tabular}{c | @{}c@{ }c@{ }c@{}} % trim={left lower right upper}
\toprule
& \multicolumn{3}{c}{ Ratio }
\\
Noise & 23.0 & 46.0 & 92.0
\\\midrule
\begin{tabular}{c}MAJ \\ $p=0.5$\end{tabular}
 & \includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=3,cpws=0.5,cti=1,cpi=0.0},inter_ws_size_ratio={23.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=3,cpws=0.5,cti=1,cpi=0.0},inter_ws_size_ratio={46.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=3,cpws=0.5,cti=1,cpi=0.0},inter_ws_size_ratio={92.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
\\\hline
\begin{tabular}{c}CYC \\ $p=0.5$\end{tabular}
& \includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=2,cpws=0.5,cti=1,cpi=0.0},inter_ws_size_ratio={23.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=2,cpws=0.5,cti=1,cpi=0.0},inter_ws_size_ratio={46.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=2,cpws=0.5,cti=1,cpi=0.0},inter_ws_size_ratio={92.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
\\\hline
\begin{tabular}{c}UAR \\ $p=1$\end{tabular}
& \includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=1,cpws=1.0,cti=1,cpi=0.0},inter_ws_size_ratio={23.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=1,cpws=1.0,cti=1,cpi=0.0},inter_ws_size_ratio={46.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=1,cpws=1.0,cti=1,cpi=0.0},inter_ws_size_ratio={92.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
\\\hline
\begin{tabular}{c}MAJ \\ $p=1$\end{tabular}
& \includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=3,cpws=1.0,cti=1,cpi=0.0},inter_ws_size_ratio={23.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=3,cpws=1.0,cti=1,cpi=0.0},inter_ws_size_ratio={46.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=3,cpws=1.0,cti=1,cpi=0.0},inter_ws_size_ratio={92.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
\\\hline
\begin{tabular}{c}CYC \\ $p=1$\end{tabular}
& \includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=2,cpws=1.0,cti=1,cpi=0.0},inter_ws_size_ratio={23.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=2,cpws=1.0,cti=1,cpi=0.0},inter_ws_size_ratio={46.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
&
\includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=2,cpws=1.0,cti=1,cpi=0.0},inter_ws_size_ratio={92.0},explore_method={expl,eps=0.1},/cdf_notitle.pdf}
\\\bottomrule
\multicolumn{4}{c}{
		\begin{subfigure}[t]{\textwidth}
			%\hspace{-1.3cm} for 1.2
    \includegraphics[width=\textwidth,trim={0 0 0 0},clip]{figs/cdfs/legends/legend_Lambda=8.pdf}
		\end{subfigure} }
\end{tabular}
\caption{Cumulative distribution functions (CDFs) for all evaluated algorithms, against different noise settings and warm start ratios in $\cbr{23.0,46.0,92.0}$. All CB algorithms uses $\epsilon$-greedy with $\epsilon=0.1$. In each of the above plots, the $x$ axis represents scores, while the $y$ axis represents the CDF values.}
\label{fig:cdfs-eps=0.1-5}
\end{figure}

\begin{figure}[H]
	%\vskip -100pt
\centering
\begin{tabular}{c | @{ }c@{}} % trim={left lower right upper}
\toprule
& \multicolumn{1}{c}{ Ratio }
\\
Noise & 184.0
\\\midrule
\begin{tabular}{c}MAJ \\ $p=0.5$\end{tabular}
 & \includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=3,cpws=0.5,cti=1,cpi=0.0},inter_ws_size_ratio={2.875},explore_method={expl,eps=0.1},/cdf_notitle.pdf}

\\\hline
\begin{tabular}{c}CYC \\ $p=0.5$\end{tabular}
& \includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=2,cpws=0.5,cti=1,cpi=0.0},inter_ws_size_ratio={2.875},explore_method={expl,eps=0.1},/cdf_notitle.pdf}

\\\hline
\begin{tabular}{c}UAR \\ $p=1$\end{tabular}
& \includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=1,cpws=1.0,cti=1,cpi=0.0},inter_ws_size_ratio={2.875},explore_method={expl,eps=0.1},/cdf_notitle.pdf}

\\\hline
\begin{tabular}{c}MAJ \\ $p=1$\end{tabular}
& \includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=3,cpws=1.0,cti=1,cpi=0.0},inter_ws_size_ratio={2.875},explore_method={expl,eps=0.1},/cdf_notitle.pdf}

\\\hline
\begin{tabular}{c}CYC \\ $p=1$\end{tabular}
& \includegraphics[width=0.29\textwidth,valign=c,trim={0 0 0 0},clip]{figs/cdfs/no_agg/corruption={st,ctws=2,cpws=1.0,cti=1,cpi=0.0},inter_ws_size_ratio={2.875},explore_method={expl,eps=0.1},/cdf_notitle.pdf}

\\\bottomrule
\multicolumn{2}{c}{
		\begin{subfigure}[t]{\textwidth}
			%\hspace{-1.3cm} for 1.2
    \includegraphics[width=\textwidth,trim={0 0 0 0},clip]{figs/cdfs/legends/legend_Lambda=8.pdf}
		\end{subfigure} }
\end{tabular}
\caption{Cumulative distribution functions (CDFs) for all evaluated algorithms, against different noise settings and warm start ratios in $\cbr{184.0}$. All CB algorithms uses $\epsilon$-greedy with $\epsilon=0.1$. In each of the above plots, the $x$ axis represents scores, while the $y$ axis represents the CDF values.}
\label{fig:cdfs-eps=0.1-6}
\end{figure}

